Towards Activity Context using Software Sensors

Service-Oriented Computing delivers the promise of configuring and reconfiguring software systems to address user's needs in a dynamic way. Context-aware computing promises to capture the user's needs and hence the requirements they have on systems. The marriage of both can deliver ad-hoc software solutions relevant to the user in the most current fashion. However, here it is a key to gather information on the users' activity (that is what they are doing). Traditionally any context sensing was conducted with hardware sensors. However, software can also play the same role and in some situations will be more useful to sense the activity of the user. Furthermore they can make use of the fact that Service-oriented systems exchange information through standard protocols. In this paper we discuss our proposed approach to sense the activity of the user making use of software.

==> eptcsdata.tex <==
\providecommand{\event}{M.H. ter Beek (Ed.): Young Researchers Workshop\\
on Service-Oriented Computing 2009 (YR-SOC'09).
}
\providecommand{\volume}{2}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{27}
\providecommand{\eid}{3}

